Reinforcement Learning for Adaptive Routing

Reinforcement learning means learning a policy--a mapping of observations into actions--based on feedback from the environment. The learning can be viewed as browsing a set of policies while evaluating them by trial through interaction with the environment. We present an application of gradient ascent algorithm for reinforcement learning to a complex domain of packet routing in network communication and compare the performance of this algorithm to other routing methods on a benchmark problem.

==> fig/my6x6res <==
# results for my6x6.net after 10000 with interreport 1000 aver over 5 runs 
# Load BEST  LEARN  BESTLOAD     POSE \eta.001 
0.1  6.      6.1     6.05        7.1
1.   6.5     6.8     6.45        8.03
1.5  7.5     8.5     7.2         8.45
1.8   16     12       10         8.8
2.   530.    22.      154        9.81
2.2  530     70       400        10.1
3.   530.    450      500        13. 

# set yrange [4:18]
# set data style lines
# set key left box
# pl 'my6x6res' u 1:2 t "Best", 'my6x6res' u 1:3 t "Learn", 'my6x6res' u 1:4 t "BestLoad", 'my6x6res' u 1:5 t "PoSe"

==> fig/res6x6 <==
# results for 6x6.net after 10000 with interreport 1000 aver over 5 runs 
# Load BEST  LEARN  BESTLOAD     POSE \eta.001 
0.1  6.      6.1     6.05        7.1*
1.   6.5     6.3     6.2        8.03
1.5  7.5     6.8     6.6        8.55
1.8  7.8     7.7     6.9        8.65
2.   9.      8.      7.4        9.71
2.2  9.5     8.7     7.7        10.5
3.   530.    18      11.5        13.
3.5  1000    120     18          20
4.   1000    280     251         40

# set yrange [4:18]
# set data style lines
# set key right bottom box
# set xlabel "Load" 0
# set ylabel "Average delivery time" 0
# pl 'res6x6' u 1:2 t "Best", 'res6x6' u 1:3 t "Q-route", 'res6x6' u 1:4 t
# "BestLoad", 'res6x6' u 1:5 t "GAPS" lt 4 lw 3


